Seamless Website Fingerprinting in Multiple Environments

Website fingerprinting (WF) attacks identify the websites visited over anonymized connections by analyzing patterns in network traffic flows, such as packet sizes, directions, or interval times using a machine learning classifier. Previous studies showed WF attacks achieve high classification accuracy. However, several issues call into question whether existing WF approaches are realizable in practice and thus motivate a re-exploration. Due to Tor's performance issues and resulting poor browsing experience, the vast majority of users opt for Virtual Private Networking (VPN) despite VPNs weaker privacy protections. Many other past assumptions are increasingly unrealistic as web technology advances. Our work addresses several key limitations of prior art. First, we introduce a new approach that classifies entire websites rather than individual web pages. Site-level classification uses traffic from all site components, including advertisements, multimedia, and single-page applications. Second, our Convolutional Neural Network (CNN) uses only the jitter and size of 500 contiguous packets from any point in a TCP stream, in contrast to prior work requiring heuristics to find page boundaries. Our seamless approach makes eavesdropper attack models realistic. Using traces from a controlled browser, we show our CNN matches observed traffic to a website with over 90% accuracy. We found the training traffic quality is critical as classification accuracy is significantly reduced when the training data lacks variability in network location, performance, and clients' computational capability. We enhanced the base CNN's efficacy using domain adaptation, allowing it to discount irrelevant features, such as network location. Lastly, we evaluate several defensive strategies against seamless WF attacks.

==> equations/eq_501_precision.tex <==
\begin{equation}
    rec = tp/(tp + fn)
\label{eq:precision}
\end{equation}

==> equations/eq_502_recall.tex <==
\begin{equation}
    rec = tp/(tp + fn)
\label{eq:recall}
\end{equation}

==> equations/eq_503_accuracy.tex <==
\begin{equation}
    prec = (tp + tn)/(tp + tn + fn + fp) \cite{prec-acc-recall_towards}
\label{eq:accuracy}
\end{equation}

==> figures_text/000_fig_samp.tex <==

\begin{figure*}[ht!]
\begin{center} 
  \begin{tabular}{cc}
  \includegraphics[width=8cm]{figures/comp_MAT_s100_snr30_8psk_r20M_2_iq_r4.png} & 
  \includegraphics[width=8cm]{figures/comp_GNU_s100_snr30_8psk_r20M_2_iq_r3.png} \\
   (A) MATLAB & (B) GNU Radio  \\ 
  \end{tabular}
  \end{center}
\caption{8PSK Constellation Plots for 100 IQ Pairs }
\label{fig:const_plot_8psk}
\end{figure*}


\begin{figure}[!ht]
\centering
\includegraphics[width=14cm]{figures/network_traffic_diagram_r2.png}
\caption{Network traffic Setup}
\label{fig:network_traffic_setup}
\end{figure}

==> figures_text/200_network_traffic_setup.tex <==

\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/network_traffic_diagram_r7.png}
\caption{Diagram of Network Setup}
\label{fig:network_traffic_diagram}
\end{figure}

==> figures_text/500_fig_web_acc_vs_num.tex <==

\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/acc_website_20k_r6.png}
\caption{Number of Sites vs Classification Accuracy}
\label{fig:web_acc_vs_num}
\end{figure}



==> figures_text/500_fig_web_acc_vs_num_3.tex <==
% Confusion Matrices
\begin{figure*}[ht!]
%\centering
\begin{tabular}{ccc}
\includegraphics[width=6cm]{figures/acc_website_10k_r4.png}\hfill & 
\includegraphics[width=6cm]{figures/Graph_placeholder.jpeg} &
\includegraphics[width=6cm]{figures/Graph_placeholder.jpeg}  \hfill \\ 
(A) Number of sites vs accuracy  &  (B) Number of samples vs accuracy  & (C) Precision, Recall and Accuracy\\ 
10 Million Packets &   & 
\end{tabular} 
\caption{Number of sites vs Accuracy}
\label{fig:web_acc}
\end{figure*}

==> figures_text/505_fig_web_prec-acc-recall.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/website_prec-recall_f1_CNN_20k_r3.png}
\caption{Precision, Recall, and Accuracy for each website}
\label{fig:web_prec-acc-recall}
\end{figure}

==> figures_text/510_fig_samples_vs_acc.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/website_samples_vs_acc_r10.png}
\caption{Number of Samples vs. Classification Accuracy}
\label{fig:web_samples_vs_acc}
\end{figure}

==> figures_text/511_fig_web_samp_acc_trend.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/website_samples_vs_acc_r11.png}
\caption{Number of Samples vs. Classification Accuracy}
\label{fig:web_samples_vs_acc_trend}
\end{figure}

==> figures_text/fig_web_acc_comb.tex <==
%--------------------------------------------------------
% Confusion Matrices
\begin{figure*}[t!]
%\centering
\begin{tabular}{ccc}
(A)  Number of Sites vs. Accuracy  &  (B) Number of Sites vs. Accuracy  & (C) Varied Number of Packets vs. \\ 
    (20 Million Samples)                & (New Web Page Data)          &  Classification Accuracy\\
\includegraphics[width=5.5cm]{figures/website_num_vs_acc_r10.png}\hfill & 
\includegraphics[width=5.5cm]{figures/web_acc_num_sites_train2_test3-1_r1.png}\hfill & 
\includegraphics[width=5.5cm]{figures/website_samples_vs_acc_r10.png}\hfill \\  

\end{tabular} 
\caption{Classification Accuracy for individual websites}
\label{fig:web_acc_comb}
\end{figure*}


==> figures_text/fig_web_acc_comb_2.tex <==



\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/website_num_vs_acc_r10.png}
\caption{Number of Samples vs. Classification Accuracy for 20 Million Packets per Website}
\label{fig:web_samples_vs_acc}
\end{figure}


\begin{figure}[!ht]
\centering
\includegraphics[width=8.5cm]{figures/web_acc_num_sites_train2_test3-1_r1.png}
\caption{Number of Samples vs. Classification Accuracy: NN Response to Aged Data}
\label{fig:web_samples_vs_acc_new_data}
\end{figure}


==> notes_extra/000_notes_edits.tex <==
\section{TO DOs and OUTLINE:}
Notes on the distributions: 
https://jamboard.google.com/d/1-S8eZYmveNUd3LQDQ75PvSexq8jByqHHw8bTQVH4VN4/edit?usp=sharing
\\
{\bf DUE: Thursday, September 14, 2023} 
\\
Make a list of the graphs we want to share 
\\
Experiments and Results:
\begin{enumerate}
\item{1}. Maximum accuracy using all data: 95\% accuracy. DONE 
\item{2}. Train on 3 sites test on 1 DONE 
\item{3}.  Train on 2 sites test on 2 DONE 
\item 4. Time: Months or year later.  For 10 Websites, train on old test on new. Get 88\% with transfer learning.
\item 5. Increase training from 1K to 20K (accuracy level out after X  1K: 30\%, 2K, 5K 80\% 10K 83\% 20K 91\% ) 
     Also use fine tuning: Use other site, 1000 samples from other locations is ~78\% 
\item 6. increasing \# of websites: 5,10,20 total websites. 
\item 7. use only time samples   (time,size)   -> time, time, time   92\% 
\item 8. Use only size samples   (time,size) -> size, size, size    93\% 
\item 9. Add randomization to the size/time pairs
        Some did not drop in accuracy with randomization: Why? 
        How is it possible to get high accuracy with randomization?  Adding 10X of the standard deviation makes accuracy go to 0. {bf We could have a curve of accuracy vs number of standard deviations added: 
        For all three data sets of: (1) size only, (2) time only and (3) size + time } 
\item 10. Is accuracy bi-modal? That is, most websites are OK but some have poor accuracy? 
\item 11. Model stability. How sensitive is the accuracy of an individual web site to the seed at the start of the training? 
\end{enumerate}  

Write a description of the how fine-tuning works.  \\
Write and how the transfer learning works.
    Example with bandwidth: Normal bandwidth as a unique feature, or maximize loss and let the 
       network figure out which features to ignore vs. which to pay attention to. \\

       Contact He Zhu, Hao Wang about participating in the paper. \\




==> notes_extra/1000_notes_text.tex <==
\section{Reliability of Synthetic Network Data Generation}
A classic study by Alessio Botta et. al. showed that generation of synthetic traffic is not always representative of real network traffic and may not follow the proper protocols. The work argues that the synthetic generation models are limited by off the shelf hardware, open source software, and the host generator's traffic status.  \cite{botta_traffic_gen} 

There are various type of Network Traffic Generators and they can usually be divided into the following categories: Application Traffic, Flow level traffic, packet traffic, and closed loop and multilevel traffic. MGEN is considered packet traffic generator software. \cite{botta_traffic_gen} 

%since it enables users interact with mulitple layers of the protocol stack including sessions, network characteristics, connections and session. \cite{botta_traffic_gen} 

Botta et. al. found that the the achievable packet and bit rate from the models were a lot smaller than the requested rates. Additionally after achieving their max some generator such as RUDE/CRUDE decrease the packet rate while others such as MGEN remain at the max capacity. \cite{botta_traffic_gen} To add to this, their works also demonstrated that the Inter Departure Time (IDT) the generated traffic was very different from that of realistic traffic.  Moreover their studies confirmed that eternal resources that the require the operating machine's CPU also impact logging, time sampling, and calculations of the packet generator.  \cite{botta_traffic_gen} 


%\input{figure_text/fig_net_set}

%\noindent \textbf{Synthetic Data} \\
%The synthetic data will be generated by using MGEN software with the following distributions: Poisson, burst, and periodic. We will be using Poisson distributions because they are commonly used in network traffic models. Bursts distributions are included burst traffic is often exhibited in real network traffic patterns \cite{cs-wustl-net-traffic}.  Periodic distributions are included because of their common usage in Network Time Protocol, Akamai CDN, and some malicious applications \cite{haffey}. 



\subsection{Traffic Generation}
We used the networks to classify data based on two type of criteria: application type and website address. The data generation technique for each is described in the sections below. 

For our application data we observed the following types of applications SCP data transfer (SCP), YouTube video downloads (YTBE), and Website browsing (WEB).  For the SCP data, we sent files over the RUNet server and observed the packet information.  For the YTBE data videos video were download via youtube-downloader.com while we monitor the traffic over the Mellanox port. For the WEB data, we use puppeteer to visit websites and scrape all the links. Then we filter for links with the same domain and visit the new links. We repeat this process until we have visited 20,000 links. 

\subsubsection{Data Formatting}
Next we, transfer the PCAP files to another directory.  We use a python script to filter the PCAP files and extract the packet timing and length information. The final step entails converting the data into a binary file for input into neural networks. The data is formatted into 32 floating-point values with interleaved packet and timing information.   All files sizes are at least 77 MB which allows us to collect a minimum of 10,000 samples per file, which is approximately 10 million packets. \\







==> notes_extra/2000_latex_notes.tex <==
%Including images across both columns
\begin{figure*}[htp]
\centering
\includegraphics[width=.3\textwidth]{i/houghtrain.png}\hfill
\includegraphics[width=.3\textwidth]{i/houghframe.png}\hfill
\includegraphics[width=.3\textwidth]{i/houghspace.png}

\caption{default}
\label{fig:figure3}

\end{figure*}

==> tables/600_table_application.tex <==

\begin{table}[!h]
    \centering
    \begin{tabular}{|c | c | c |}
    \hline
    \textbf{Label} & \textbf{Application}   & \textbf{Data type}\\  \hline
     SCP           &   SCP                  & Downloading video data over SCP  \\ \hline
     %TIKTOK        &   Tik Tok Server       & Accessing  video data over TikTok server  \\ \hline
     YTBE        &   YouTube Downloader   & Downloading video data using youtube.dl  \\ \hline
     %MINCRFT       &   Minecraft Server     & Accessing information via Minecraft server \\ \hline
     WEB            &   The internet        & Accessing various websites  \\ \hline

    \end{tabular}
    \caption{Ethernet Traffic Application Data Types} \\
    \label{tab:app_data_list}
\end{table}

==> tables/601_table_website_list.tex <==


\begin{table}[!h]
    \centering
    \begin{tabular}{|c | c |}
    \hline
    \textbf{Label} & \textbf{Web Address} \\  \hline
     brit            &   www.britannica.com       \\ \hline
     cnn            &   www.cnn.com        \\ \hline     
     ebay            &   www.ebay.com        \\ \hline
     foxn            &   www.foxnews.com        \\ \hline
     nfl            &   www.nfl.com        \\ \hline
     nyt            &   www.nytimes.com        \\ \hline
     rddt            &   www.reddit.com        \\ \hline
     trgt            &   www.target.com        \\ \hline
     yelp            &   www.yelp.com        \\ \hline
     yho            &   www.yahoo.com        \\ \hline
    \end{tabular}
    \caption{Ethernet Traffic Application Data Types}
    \label{tab:website_list}
    \vspace*{-4mm}
\end{table}


==> tables/602_table_website_by_number.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{|c | c |}
    \hline
    \textbf{Number of sites} & \textbf{Sites} \\  \hline
     2      &   brit cnn       \\ \hline
     3      &   brit cnn ebay       \\ \hline
     4      &   brit cnn ebay foxn        \\ \hline
     5      &   brit cnn ebay foxn nfl       \\ \hline
     6      &   brit cnn ebay foxn nfl nyt        \\ \hline
     7      &   brit cnn ebay foxn nfl nyt rddt     \\ \hline
     8      &   brit cnn ebay foxn nfl nyt rddt trgt       \\ \hline
     9      &   brit cnn ebay foxn nfl nyt rddt trgt yelp   \\ \hline
     10     &   brit cnn ebay foxn nfl nyt rddt trgt yelp yho  \\ \hline
    \end{tabular}
    \caption{Website Grouping by numbers}
    \label{tab:website_list_num}
\end{table}


==> text/050_Abstract.tex <==
\noindent \textbf{ \textit{Abstract:} 
 We quantify the classification accuracy of Neural Networks (NNs) to specific websites using only the packet size and difference in inter-packet arrival time, which are easily observable via passive attackers in the network. Our flow classification work with NNs is unique in that we do not classify traffic by application type. Rather, we observe the accuracy of various NNs classifying specific websites using HTTP traffic over TCP. We test a diverse set of neural network structures including a fully connected network (FCN), a convolutional neural network (CNN), a long short-term memory network (LSTM), and an autoencoder network (AE). We found that CNNs consistently had the highest accuracy, typically 80-90\% when using 20 million packets as training data. We suspect that individual websites generate unique traffic patterns which are discoverable using NN techniques. Our work has important privacy implications. In particular, our work supports that both packet sizes and inter-packet timing must be randomized to obtain strong web browsing privacy. Many privacy preserving techniques, such as VPNs, will require additional enhancements.} \\

%%The rapid growth in technology has lead to overloaded servers, security threats, and network traffic collisions. In order to mitigate these issues, much research has been devoted to network traffic classification. Unfortunately,  most studies involve using a complex feature set with multiple parameters. Additionally, much of this work focuses classifying applications rather than websites. Our research uses neural networks to identify specific websites, using only the packet size and inter-arrival time. This simplified feature space is easily accessible and unencrypted. The information is available even if the data payload is encrypted or the user applies methods to obfuscate the ip address or payload data. We provide insight into the website classification through a diverse set of neural network structures including a fully connected network (FCN), a convolutional neural network (CNN), a long short term memory network (LSTM), and an autoencoder network (AE). Rather than using a single neural network structure, such as a CNN, we provide a robust view of multiple machine learning techniques. Our work shows that as the number of website increases the classification accuracy of the networks decreases.  In this work we attained accuracy levels greater than 82\% when distinguishing between 10 unique websites.  Additionally we review the impact of varied dataset sizes on classification accuracy.  \\

\noindent\textit{\textbf{Keywords:} Machine Learning, Deep Learning, Neural Networks, Website classification, network, traffic classification, CNN, LSTM, Dense Network, FCN, MLP, Multilayer perceptron, Autoencoder, packets, inner-arrival time, packet length}


==> text/075_Outline.tex <==

\section{Outline} 

(Internal notes, will remove later) 

This is the paper outline and list of datasets 

ISPs and their locations:

Vultr:
\hspace{0.25in} London, Chicago, Miami

Rutgers; 
 \hspace{0.25in}  New Brunswick 

Geni: 
\hspace{0.25in} Univ. of Washington (Seattle) 

List of Websites: 

{\bf What is the accuracy under different scenarios assuming a privacy attack? }

What is the combination of training and testing sets? 

One end of the spectrum is to combine all the data in 1 very large set and see what is the accuracy 

\begin{itemize}
\item Large ISP will all the data: Mix up all the data and do 10-fold cross validation.

\item Take training from 1 location and apply to a different location in pairwise blocks: Example: Training is Miami, testing is Rutgers, training is London, testing is Chicago .. 

\item combinations of locations: 3 locations for training, 1 for testing, example: Rutgers + London + Chicago, testing is Miami:  

\item What are the impacts of X on Accuracy? Where is factor is: \\
- Maximum training size: Overall best accuracy combining all the data from all the sites and locations \\
- Different Locations: When training and testing locations are different \\ 
- Increasing packet count: number of packets in the training set \\
- Longer timescales: long time between training and test \\ 
- Host environment: Type of sites in training vs testing: (cloud, server, home-network)? \\
- number of websites: number of sites in the training and testing sets? \\
- Using Domain Adaptation: Domain adaptation? \\
- Only Time: Just using time?\\
- Only Size: Just using size? \\
- Protecting Privacy: Adding randomization? \\
 -- randomizing packet sizes and times\\
--- adding extra traffic? \\ 
\end{itemize}

==> text/105_background.tex <==
\section{Related Work}
\label{sect:Background_eth}
Space limitations preclude us from providing a full treatment of the vast related works on using Machine Learning (ML) for network traffic classification. We thus include a sample of the most closely related studies to illustrate prior efforts and show our unique contributions to flow classification. 

One related work used a feature-rich set comprised of port server number, number of bytes, number of data packets, packet inter-arrival time, and additional information~\cite{moore_network_traffic} to distinguish between different types of network traffic. The results showed over 98\% classification accuracy for a test set including FTP, P2P, database, and website applications. A drawback of this approach is that there are several features to consider and the optimal combination for these features varies in different scenarios. Additionally, the research limits the neural network structure to a fully connected network only. 

A second very related study on ML for traffic classification used CNNs and Recurrent Neural Networks in their approach\cite{lopez-2017-network}. This work employed a feature space of IP addresses, port numbers, and transport protocols. The researchers identified 15 common services with over 99\% accuracy. Their service labels included YouTube, HTTP, Telnet, Apple, and Office 365. Although the accuracy of the work is impressive, it involves using network features that may not always be readily available.

A third related study used packet length, inter-arrival times, flow direction, flow volume, and protocol for the feature space~\cite{williams2006preliminary}. The work classified traffic flow parameters with over 90\% accuracy.  The benefit of the work was its high accuracy.  However, the feature space is more complex than our research. 

Some research included a more simplified feature space for traffic classification. In fact, one study used only the packet payload for machine learning network classification \cite{lim_packet_2019}. The work showed that processing network data in multiple steps can increase classification accuracy. Here, the data packet payload was pre-processed to create deep learning datasets.  The NNs included CNN and Residual (ResNet) structures.  The results  showed accuracy levels above 96\%.  Also, the outcome indicated that the ResNet network outperformed the CNN. 

Another promising study by Shahbaz Rezaei et. al. also applied multi-step data processing for network traffic classification~\cite{google_rezaei_2018achieve}. They used a semi-supervised machine learning approach to distinguish between Google Drive, YouTube, Google Docs, Google Search, and Google Music.  In their work, they pre-trained part of the network on unlabeled data. This trained data was then fed into a new network model with labeled data.  They used timing information of packets as the feature space. They attained over 90\% accuracy for script-generated traffic and approximately 81\% for human-generated traffic. This work shows that different machine learning techniques can be used to classify web applications.  Unfortunately, this dataset was limited to 5 Google-based web applications rather than distinct websites.  

Many researchers realized some traffic information such as the data payload may not always be accessible and have proposed ML techniques that do not require this information. For example, Tom Auld, Andrew Moore, et. al. used packet header content without payload information for traffic classification. Their feature set included packet inter-arrival time, the packet size of control fields, total number of packets, payload size, and other information. They used Bayesian neural networks with supervised learning to separate the traffic into 10 categories ranging from database to multimedia to "www". They achieved an average accuracy of 68.8\% for all 10 classes~\cite{auld_2007_bayesian}.




==> text/2000_testing_stuff.tex <==
\begin{figure*}[t!]
\centering
\begin{tabular}{cc}
\includegraphics[width=5.5cm]{images/SNR_vs_Acc_GRID_1k_samp_node18-1_dist-comp_CAT_no-match_r1.png}\hfill & 
\includegraphics[width=5.5cm]{images/SNR_vs_Acc_GRID_1k_samp_node18-1_dist-comp_LSTM_no-match_r1.png}  \\ 
(FCNN) & (CNN) \\ 
\end{tabular} 
\caption{SNR vs Accuracy}
\label{fig:figure3}
\end{figure*}


\begin{figure*}[t!]
\centering
\begin{tabular}{cc}
\includegraphics[width=5.5cm]{images/SNR_vs_Acc_GRID_1k_samp_node18-1_dist-comp_CAT_no-match_r1.png}\hfill & 
\includegraphics[width=5.5cm]{images/SNR_vs_Acc_GRID_1k_samp_node18-1_dist-comp_LSTM_no-match_r1.png}  \\ 
(FCNN) & (CNN) \\ 
\end{tabular} 
\caption{SNR vs Accuracy}
\label{fig:figure3}
\end{figure*}


\begin{figure*}[t!]
\centering
\begin{tabular}{ccc}
\includegraphics[width=5.5cm]{i/houghtrain.png}\hfill & 
\includegraphics[width=5.5cm]{i/houghframe.png}\hfill & 
\includegraphics[width=5.5cm]{i/houghspace.png}  \\ 
(A) & (B) & (C) \\ 
\end{tabular} 
\caption{default caption text is here }
\label{fig:figure3}
\end{figure*}


==> text/200_neural_networks.tex <==
\section{Neural Networks}
\label{sect:classification_nets }
We investigated several NN types, in particular CNN, FCN, LSTM, and AE neural networks. We selected these networks because of their varying structures and diversity in operation. For example, CNNs are extremely useful in image recognition while AEs are often used to denoise data.  In this section, we provide some background and describe our implementations of these networks. \\

\subsection{Fully Connected Network (FCN)}
One common neural network structure is the multi-layer perceptions (MLPS) or fully connected network (FCN). In FCNs each node is "connected" to all the nodes in the previous layer~\cite{Janke}. Historically, FCNs were known for having longer training times than other networks. However, developments in software libraries and computational resources have decreased the timing of FCNs. Moreover, some studies show that the FCNs have comparable accuracy to other networks~\cite{burns2021_sig_gen, burns2021}.  Our FCN contains four fully connected layers with 400, 200, 100, and 50 nodes, followed  by a "dropout" layer.   The output layer is a fully connected dense layer with \textit{N} nodes, where \textit{N} refers to the number of classes. The dropout and output layer is identical for all four neural networks. 

\subsection{Convolutional Neural Network (CNN)}
%\noindent \textbf{Convolutional Neural Network (CNN)} \\
Convolutional neural networks (CNNs) are vert popular. They are used in applications ranging from image classification to speech recognition to automatic modulation recognition~\cite{Sharifzadeh, EEGNet_Lawhern}. CNNs function by applying sliding filters to the data and producing a "convolved" output~\cite{cnns-medium}.   For 3d filters, the outputs are 2d matrices of weights and parameters.  The size and dimensions of these are adjusted through the max pooling and upsampling layers of the network~\cite{upsampling_corner, cnns-medium, maxpool-computerscience}.  The CNN network of this project contains 6 2D convolutional layers interleaved with 3 max pooling layers and 3 upsampling layers.  The convolutional layers have filters ordered as follows: 32, 16, 8, 8, 16, and 32.  The latter half of the network consists of two dense layers with 512 and 256 nodes. The last layers of the network are the dropout and a fully connected output layer with \textit{N} nodes. 

\subsection{Autoencoder (AE)}
%\noindent \textbf{Autoencoder (AE)} \\
Autoencoders (AEs) are generative models containing two main components: an encoder and a decoder. The encoder learns hidden features in the input data and compresses the information into a smaller feature set~\cite{AE-keras-tutorial}. The decoder "reconstructs" the data from a compressed model~\cite{toward-auto-simple, AE-keras-tutorial}. AEs are beneficial since they reduce the dimensionality of feature spaces~\cite{ae-cyber-yoursefi}.  AEs have been used in cyber security, anomaly detection, automatic wireless technology recognition, and other applications~\cite{ae-cyber-yoursefi, ae-camelo, ae-tan}.  The encoder of our AE has 4 fully connected dense layers with 256, 128, 64, and 32 nodes.  The decoder is a mirrored structure of the encoder with dense layers of 32, 64, 128, and 256 nodes.  The decoder is succeeded by a dropout and fully connected output layer. 

\subsection{Long Short-Term Memory (LSTM)}
%\noindent \textbf{Long Short Term Memory Network (LSTM)} \\
Long short term memory networks (LSTMs) as classic time recursive neural networks~\cite{Li-LSTM}.   This means that the model uses prior content along with the current data for each layer~\cite{Ney-LSTM-Lan}.  LSTMs are ideal for data containing delays and time series~\cite{Li-LSTM}. Our LSTM network consists of two LSTM layers with 32 filters, a dropout layer, and a fully connected dense layer with \textit{N} nodes.  As a note, this network is relatively shallow due to timing constraints and computational resource limitations. For more information regarding this please refer to ~\cite{burns2021_sig_gen} and ~\cite{burns2021}. 







==> text/300_simulation_description.tex <==
\section{Methodology} 
\label{sect:methodology}
The focus of this research is to compare how accurately different neural networks classify website traffic with a simplified feature space. Two of the most easily accessible features of network traffic are packet inter-arrival time and length distribution. Moreover, these features are major components of network models~\cite{cs-wustl-net-traffic}.   Other features such as the payload data may be difficult to access if they are protected or encrypted.  

\subsection{Network Setup}
We collected traffic information by setting up the network shown in \ref{fig:network_traffic_diagram}. The client and server were Dell R7525 computers located at the Hill Center of Rutgers University. A Dell port 1/1/25 vlan2300 was our switch.  This high-speed switch is connected to the Mellanox ports where we collected PCAP files in one-minute intervals. There are a total of 60 files for each monitoring port and each hour the files are overwritten with new data. The \textit{eno1} port monitors traffic between the host and the RUNet network.  So, traffic from the websites is monitored here.  %The enos710 port is used to monitor the traffic from the switch.  So, synthetically generated data is monitored here.  

\input{figures_text/200_network_traffic_setup}

\subsection{Traffic Generation}
Our approach to generating web traffic is intended to be as realistic as possible. As such, we used the puppeteer framework to control a Chrome web browser~\cite{puppeteer}. This ensures we will generate all the traffic, including scripts and advertisements. To model a person browsing, we view the website as a graph of pages connected by hyperlink URLs within a single web domain. We start at the top level root page and follow a randomly picked child link pointing within the same web domain, and repeat this process until we reach a leaf page. We then return to the main page, repeating the process of following random children until we generate sufficient traffic. The websites are listed in \ref{tab:website_list}. All the generated traffic is monitored via the Mellanox ports discussed in Section \ref{sect:methodology}.

\input{tables/601_table_website_list}

\subsection{Data Formatting}
After collecting the saved packets to files, a script filters them to only include packet timing and length information. We converted the packet files into binary input files for the neural networks. Each packet is reduced to a pair of 32 floating-point values, one for the size and one for the delay from the previous packet encoded in microseconds. Each processed trace file is 77 MB, which at 8 bytes per packet (2 values), is 9.6M packets per site. 


 



==> text/400_transfer_learning.tex <==
\subsection{Transfer Learning}

Put in the figure and equations on the transfer learning.

and decribe the training process.



==> text/500_Experiment_Results.tex <==

\section{Experiment Results and Discussion}
\label{sect:experiments}
%\input{figures_text/500_fig_web_acc_vs_num}
We examined 10 websites using the packet length and timing collected over the Rutgers University Network. With these 10 sites, the sample size was over 100 million packets in total. This allowed us to observe the response of the networks as we varied the number of sites and the sample size. The next sections will discuss our results. 

\subsection{Accuracy Analysis for Website Traffic} 
For our accuracy analysis we examined 3 factors: (1) the number of websites, (2) the NN response to aged website traffic, and (3) the impact of the varied sample sizes.  

%\subsubsection{Classification Accuracy with increasing websites }
\textbf{Number of Websites: }
We observed the classification accuracy of the networks as the number of websites increased. This is vital because it indicates how robust each network is in classifying multiple websites.  The CNN network has the best performance overall with an accuracy of 82\% for 10 websites. The LSTM has the worst performance with less than 25\% accuracy for 10 websites.  (As a note, part of the poor performance is likely due to the shallow structure of the network. For more details regarding this, please refer to Section \ref{sect:methodology}.)  All networks show a decline in accuracy as the number of sites increases, which aligns with our expectations. The accuracy results are shown in Fig. \ref{fig:web_samples_vs_acc}. Due to time limitations, we were only able to collect packets for 10 websites. 

%\input{tables/602_table_website_by_number} 
%\subsubsection{NNs Response to New Data}
\textbf{NNs Response to Aged Traffic: }
Websites are constantly being updated with new information.  For example, amazon.com updates their pages with new product listings regularly. Thus, it is important to determine how the NNs perform as the training data ages. We trained on website traffic collected in April of 2022 (Dataset 2) and tested on traffic collected in August of 2022 (Dataset 3).  We found that the network had a 10\% drop in accuracy over this four-month period, most likely due to updated web pages. The results are displayed in Fig. \ref{fig:web_samples_vs_acc_new_data}
\input{figures_text/511_fig_web_samp_acc_trend}

%\subsubsection{Varied Sample Size}
\textbf{Varied Sample Size: }
We also observed the impact of varying training sample size on classification accuracy. As expected, increasing the training sample size improves the overall results.  For example, the accuracy of CNN network improves by approximately 5\%  from 10 million to 20 million packets. Based on the data we suspect that additional samples would continue to increase the accuracy. Due to time constraints, we were not able to attain additional packet samples.  However, we ran a linear regression curve on a logarithmic scale  to forecast the accuracy with additional samples. The model indicates that the CNN could reach 94\% accuracy at approximately 40 million samples. Fig. \ref{fig:web_samples_vs_acc_trend} summarizes our results. For each neural network, the actual results are depicted in a solid line while the linear regression model is shown in a dashed line of the same color. 
%\input{figures_text/510_fig_samples_vs_acc}
\input{figures_text/fig_web_acc_comb_2}

Based on the results in Fig. \ref{fig:web_samples_vs_acc} we hypothesize that as more websites are added, the overall accuracy will decrease. However, if there is a training data is increased, we suspect that the networks, particularly the CNN, will still maintain relatively high results. With enough training data, we believe that the networks can be scaled up to predict 100s of websites. 

\subsection{Precision, Recall, and F1 score} 
While accuracy informs us of the overall of how many times the network model was correct \cite{precision-recall_mage} the precision, recall, and $F_1$ score provide a deeper view into the network's performance for each website. We used our best-performing ML model, the CNN network, to observe the metrics for each website.  Precision measures the false positive error rate while recall measures the false negative rate~\cite{prec-acc-recall_Zeya}. The $F_1$ score is a harmonic balance between precision and recall~\cite{prec-acc-recall_Zeya}.  A high $F_1$ score indicates that the model has a low overall error rate for that particular class~\cite{prec-acc-recall_Zeya}. 

Fig. \ref{fig:web_prec-acc-recall} demonstrates the precision, recall, and $F_1$ score for each website. These results show that the neural networks classify some websites with higher accuracy than others.  For example, the F1 score of cnn is only 71\% while the brit site has an F1 score of 90\%. We also observed that some sites have a noticeable difference between the recall and precision metrics.  For instance, yho has a precision of 92\% but its recall is only 80\%.  In contrast, the nfl precision rate is higher than its recall at values of 86\% and 73\%. %We expect that as the number of website expand the variability in the metrics will increase. 

\input{figures_text/505_fig_web_prec-acc-recall}

%While accuracy informs us of the overall of how many times the network model was correct~\cite{precision-recall_mage} the precision, recall, and f1 score provide a deeper view into the networks performance for each website.  Precision, or the positive predictive value, measures how well a model predicts a specific category \cite{precision-recall_mage, precision-recall_wiki}. This can be viewed as the ratio of true positives to all positives \cite{prec-acc-recall_analytic-vidhya}.  The recall or sensitivity, measures the model's ability to detect a particular class. In order words, how well can the model predict positive cases for a class? This is the ratio of the true positives combined true positives and false negative scores.  Recall is an important metric, particularly in medical field where the objective is the detect diseases with high certainty. The precision and recall equations are displayed in \ref{eq:} and \ref{eq:}. 

%Ideally, we want to maximize both of these metrics in order to reduce false predictions

%The accuracy for each class is determined by equation \ref{} In these formulas tp, tn, fp, and fn refer to true positive, true negative, false positive and false negative respectively.  

%\input{equations/eq_503_accuracy}

%Precision ->  How many cases are actually positive among the predicted positive cases? 
%Recall --> How will can i predict the positives of a class?  --> Sensitivity


==> text/800_related_work.tex <==
\section{Related Work}

\subsection{Transfer Learning }
Transfer Learning is a machine learning paradigm that leverages knowledge learned from one domain (source domain) to improve performance in another, often related, domain (target domain). Some notable approaches and contributions in this field include\cite{zhuang2020comprehensive}


In the field of deep learning, the "pretrain-finetune" paradigm has garnered significant attention as a crucial branch of transfer learning. For instance, models like GPT-3~ \cite{brown2020language} and T5~ \cite{raffel2020exploring}, which are pretrained on large-scale text data, have demonstrated exceptional performance across various downstream tasks. However, as we began to collect diverse website data from different locations, time periods, and Internet Service Providers (ISPs), we accumulated a substantial amount of labeled data. Our objective is to amalgamate this data to train a more robust model capable of excelling in diverse contexts. We anticipate that this model will achieve high accuracy on data from these varying scenarios. Moreover, we expect it to perform well on entirely untrained new datasets using zero-shot reasoning or after fine-tuning with limited labeled data. This approach will enable us to effectively tackle diversity and complexity, thereby enhancing the model's performance and generalization capabilities.


\noindent
\textbf{Domain Adaptation}:
\label{sec:method}
Domain adaptation is a widely applied branch in the field of transfer learning, with a primary focus on addressing the disparities in data distributions across different domains. The main objective of domain adaptation is to mitigate the adverse effects of domain shifts on model performance. In our case, a domain shift becomes visible when changing the origin of the packet traffic, for example, browsing from Chicago vs. Miami. When changing the traffic source point the CNN may learn features of the first domain, as opposed other domains. Domain changes involve adjusting feature distributions or modifying models in various ways to enhance their performance on the target domain.

Currently, there has been a proliferation of models \cite{prabhu2021sentry,peng2019moment} and methods \cite{carlucci2017autodial,ganin2016domainadversarial} related to domain adaptation, especially in domains such as computer vision (CV) and natural language processing (NLP).
Among these methods, Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} have found extensive use in domain adaptation. GANs are employed to align feature distributions between domains by training a domain discriminator. This approach aids in reducing the feature discrepancies between the source and target domains, ultimately improving the model's ability to generalize on the target domain.
Additionally, when dealing with training data that encompasses multiple diverse domains, the incorporation of domain indices has proven helpful in mitigating differences among domains. This approach assists in balancing the gaps between various domains, thereby enabling better adaptation to the data of the target domain. Furthermore, certain models \cite{xu2023domainindexing,xu2023graphrelational,NEURIPS2021_45017f65} have the capability to smoothly transition between domains during continuous domain shifts\cite{wang2020continuously,liu2023taxonomystructured}, extracting common features. This is particularly significant for handling multi-domain data.
In summary, domain adaptation stands as a pivotal branch of transfer learning, primarily focused on addressing the challenges posed by domain shifts to enhance model performance on target domains.

\noindent
\subsection{Backdoor Learning }
Backdoor learning focuses on understanding and mitigating vulnerabilities associated with machine learning models that are manipulated to produce erroneous outputs when exposed to specific, crafted inputs. Based on prior research \cite{turner2019cleanlabel,li2022backdoor,Wang_2022_CVPR}, it has been demonstrated that attackers can manipulate the output of machine learning models and reduce their accuracy by injecting a small fraction of malicious data into the training dataset.

